Localization and Duality for ABJM Latitude Wilson Loops

We investigate several aspects of BPS latitude Wilson loops in gauge theories in three dimensions with $\mathcal{N}\ge 4$ supersymmetry. We derive a matrix model for the bosonic latitude Wilson loop in ABJM using supersymmetric localization, and show how to extend the computation to more general Chern-Simons-matter theories. We then define latitude type Wilson and vortex loop operators in theories without Chern-Simons terms, and explore a connection to the recently derived superalgebra defining local Higgs and Coulomb branch operators in these theories. Finally, we identify a BPS loop operator dual to the bosonic latitude Wilson loop which is a novel bound state of Wilson and vortex loops, defined using a worldvolume supersymmetric quantum mechanics.

==> Section_Matrix_Model.tex <==
\section{\label{sec:The-latitude-matrix-model}The latitude matrix model}

In this section, we attempt to derive the matrix model for the bosonic
latitude Wilson loop by supersymmetric localization. In supersymmetric localization,
one first deforms a supersymmetric Euclidean action $S$ by adding a term
$t\delta V$, where $\delta$ is a supersymmetry transformation, $V$
a positive semi-definite fermionic functional, and $t$ a positive number. The deformed partition
function, or the expectation value of a $\delta$-closed observable
$\mathcal{O}$, can be shown to be $t$-independent using the following
standard argument
\begin{align*}
\frac{d}{dt}\left\langle \mathcal{O}\right\rangle  & _{t}\equiv\frac{d}{dt}\int\mathcal{D}\Phi\mathcal{O}\exp\left(-S-t\delta V\right)\\
 & =-\int\mathcal{D}\Phi\left(\delta V\right)\mathcal{O}\exp\left(-S-t\delta V\right)\\
 & =-\int\mathcal{D}\Phi\delta\left[V\mathcal{O}\exp\left(-S-t\delta V\right)\right]\\
 & =0.
\end{align*}
Localization onto the moduli space, defined as the space of field configurations where $\delta V$ vanishes, occurs in the limit $t\rightarrow\infty$.

In verifying $t$-independence, we have assumed $\delta S=\delta\mathcal{O}=\delta^{2}V=0$.
We have also assumed that the convergence properties of the path integral
do not depend on $t$, and that the measure $\mathcal{D}\Phi$, where
$\Phi$ stands for all dynamical fields, is $\delta$-invariant, i.e.
the supersymmetry is not anomalous. If the supersymmetry generated
by $\delta$ is closed off-shell, without using the equations of motion
coming from $S$, then $\delta^{2}$ is a bosonic symmetry transformation. In this case, 
one can usually arrange for $V$ to be $\delta^{2}$ invariant. Unfortunately, off-shell closure of even a single supersymmetry transformation can
be tricky. We will deal with this difficulty in the context of the ABJM model in an ad hoc manner.

We will perform localization in two different contexts. In Section
\ref{subsec:Localization-in-the-ABJM-model} we perform localization in the ABJM model and derive a matrix model for the expectation value of the bosonic latitude Wilson loop. This calculation almost proves the conjectured form of the matrix model put forth in \cite{Bianchi:2018bke}. The only caveat is our assumption that a certain procedure can be used to close the latitude supersymmetry transformation off-shell. In Section \ref{subsec:Localization-in-a-dual-theory}, we consider an $\mathcal{N}=4$
gauge theory in the same universality class as ABJM. We
use the form of the latitude supersymmetry algebra to conjecturally
identify the operator $\mathcal{O}$ representing the bosonic latitude
loop in this IR dual theory. We then perform localization in the dual model and derive a matrix model expression for the expectation value of the dual loop operator. The matrix models for
the two theories look somewhat different, but yield the same result
for the expectation value of the loop.  This constitutes our primary
evidence for the validity of the identification of the dual loop operator.

\input{Subsection_Localization_In_ABJM}
\input{Subsection_Localization_Dual_Theory}

==> Section_Three_Sphere.tex <==
\section{\label{sec:The-latitude-on-the-three-sphere}The latitude on the three sphere}
In this section, we analyze the latitude Wilson loop conformally mapped
to the round three sphere. In Section \ref{subsec:ABJM_sphere_algebra}, we exhibit the superalgebra generated by
the latitude supercharges on the three sphere using the ABJM notation. In Section \ref{subsec:N4_standard}, we define latitude supercharges in \textit{standard} $\mathcal{N}=4$ theories: those without Chern-Simons terms. 
We show
that the latitude supercharges are related, in this context, to the supercharges used to define the topological quantum
mechanics investigated in \cite{Dedushenko:2016jxl}. We then classify
generic loop operators preserving the latitude supercharge in this class of theories. These loop operators will be used in the next section to identify
the dual of the ABJM latitude loop in a standard theory in the same universality class. Finally, in Section \ref{subsec:SQM}, we exhibit the latitude superalgebra as it acts on the supersymmetric quantum mechanics on a loop operator worldvolume. 

\input{Subsection_ABJM_Sphere_Algebra}
\input{Subsection_N4_Supercharges}
\input{Subsection_SQM}
